Learning Explainable Representations of Complex Game-playing Strategies

As part of learning to play complex games, human players develop develop abstractions for concepts and strategies of gameplay consistent with game rules to improve their performance. These concepts are applied to explain other players' actions, and to inform their own actions in-game. Understanding other players' strategies is a crucial part of such improvement, but requires time and effort. In this paper, we propose a strategy similar to human cognition for training RL agents to synthesize learned strategies and policies as executable procedures based on sequences of gameplay actions. We present methods to automatically learn such programs to play chess and to solve tasks in a grid-based environment. We show that the learned strategies produce effective actions, and can be learned from gameplay data.

==> figs/dt_progs.tex <==
\begin{figure}
    \centering
    \begin{lstlisting}
        DEF run m( WHILE c( markersPresent c) w( turnRight w) move IF c( not c( markersPresent c) c) i( turnRight move i) m)
        DEF run m( WHILE c( noMarkersPresent c) w( turnRight move w) IF c( rightIsClear c) i( WHILE c( frontIsClear c) w( move w) i) m)
        DEF run m( WHILE c( noMarkersPresent c) w( IF c( frontIsClear c) i( move i) turnRight move w) m)
        DEF run m( WHILE c( noMarkersPresent c) w( WHILE c( not c( markersPresent c) c) w( turnRight move w) w) m)
        DEF run m( WHILE c( frontIsClear c) w( turnLeft w) WHILE c( markersPresent c) w( turnRight move w) m)
        \end{lstlisting}
    \caption{The last 5 programs sampled from the decision transformer model for the stairClimber task.}
    \label{fig:dt-programs-stairClimber}
\end{figure}

==> figs/loss_mean.tex <==
\begin{figure}[htbp]
    \centering
    \begin{tikzpicture}
        \begin{axis}[xlabel={Step},ylabel={Loss}]
            \addplot table [mark=none, x=Step, y=cleanHouse, col sep=comma] {data/loss_mean.csv};
            \addlegendentry{cleanHouse}

            \addplot table [mark=none, x=Step, y=fourCorners, col sep=comma] {data/loss_mean.csv};
            \addlegendentry{fourCorners}

            \addplot table [mark=none, x=Step, y=harvester, col sep=comma] {data/loss_mean.csv};
            \addlegendentry{harvester}

            \addplot table [mark=none, x=Step, y=randomMaze, col sep=comma] {data/loss_mean.csv};
            \addlegendentry{randomMaze}

            \addplot table [mark=none, x=Step, y=stairClimber, col sep=comma] {data/loss_mean.csv};
            \addlegendentry{stairClimber}

            \addplot table [mark=none, x=Step, y=topOff, col sep=comma] {data/loss_mean.csv};
            \addlegendentry{topOff}
        \end{axis}
    \end{tikzpicture}
    \caption{Mean loss of the Decision Transformer model on each Karel task during training.}
    \label{fig:loss-mean}
\end{figure}

==> figs/loss_std.tex <==
\begin{figure}[htbp]
    \centering
    \begin{tikzpicture}
        \begin{axis}[xlabel={Step},ylabel={Loss deviation}]
            \addplot table [x=Step, y=cleanHouse, col sep=comma] {data/loss_std.csv};
            \addlegendentry{cleanHouse}

            \addplot table [x=Step, y=fourCorners, col sep=comma] {data/loss_std.csv};
            \addlegendentry{fourCorners}

            \addplot table [x=Step, y=harvester, col sep=comma] {data/loss_std.csv};
            \addlegendentry{harvester}

            \addplot table [x=Step, y=randomMaze, col sep=comma] {data/loss_std.csv};
            \addlegendentry{randomMaze}

            \addplot table [x=Step, y=stairClimber, col sep=comma] {data/loss_std.csv};
            \addlegendentry{stairClimber}

            \addplot table [x=Step, y=topOff, col sep=comma] {data/loss_std.csv};
            \addlegendentry{topOff}
        \end{axis}
    \end{tikzpicture}
    \caption{Loss standard deviation of the Decision Transformer model on each Karel task during training.}
    \label{fig:loss-std}
\end{figure}

==> tabs/hyper.tex <==
\begin{table}[htbp]
    \centering
    \caption{Hyperparameters used for training the Decision Transformer for the Karel programmatic policy synthesis task.}
    \begin{tabular}{@{}ll@{}}
        \toprule
        \textbf{Hyperparameter}   & \textbf{Value}       \\ \midrule
        Embedding dimension       & 128                  \\
        Context length ($K$)      & 50                   \\
        Activation function       & ReLU                 \\
        Batch size                & 64                   \\
        No. of attention layers   & 3                    \\
        No. of attention heads    & 2                    \\
        Dropout                   & 0.05                 \\
        Learning rate             & $1.0 \times 10^{-3}$ \\
        Weight decay              & $5.0 \times 10^{-4}$ \\
        Warm-up steps             & 200                  \\
        No. of training steps     & 200                  \\
        GRU hidden size           & 512                  \\
        GRU layers                & 1                    \\
        GRU dropout               & 0.05                 \\
        Return-to-go conditioning & 2.2                  \\
        Grad norm clip            & 0.25                 \\
        No. of eval. episodes     & 64                   \\
        Top-k\%                   & 0.01                 \\
        Max iterations            & 10                   \\ \bottomrule
    \end{tabular}
    \label{tab:hyperparams}
\end{table}

==> tabs/traj_returns.tex <==
\begin{table}[htbp]
    \centering
    \caption{Statistics for the trajectories used to train the decision transformer.}
    \begin{tabular}{@{}lllc@{}}
        \toprule
        \multirow{2}{*}{\textbf{Task}} & \multicolumn{3}{c}{\textbf{Trajectory Returns}}                                                     \\ \cmidrule(lr){2-4}
                                       & \multicolumn{1}{c}{mean}                        & \multicolumn{1}{c}{max} & \multicolumn{1}{c}{min} \\ \midrule
        cleanHouse                     & $0.10 \pm 0.00$                                 & 0.24                    & 0.1                     \\
        harvester                      & $0.09 \pm 0.08$                                 & 0.66                    & -1.26                   \\
        fourCorners                    & $0.10 \pm 0.03$                                 & 1.1                     & 0.1                     \\
        randomMaze                     & $0.16 \pm 0.08$                                 & 1.1                     & 0.1                     \\
        stairClimber                   & $0.10 \pm 0.03$                                 & 1.1                     & 0.1                     \\
        topOff                         & $0.19 \pm 0.07$                                 & 1.1                     & 0.1                     \\ \bottomrule
    \end{tabular}
    \label{tab:dt-dataset-returns}
\end{table}

==> tabs/traj_stats.tex <==
\begin{table}[htbp]
    \centering
    \caption{Statistics for the LEAPS program dataset.}
    \begin{tabular}{@{}ll@{}}
        \toprule
        Transitions    & 870,782                           \\
        Programs       & 50,000                            \\
        Program Length & $19.30 \pm 5.96\ (min=7, max=50)$ \\
        Episode Length & $17.42 \pm 4.33\ (min=5, max=30)$ \\ \bottomrule
    \end{tabular}
    \label{tab:dt-dataset-stats}
\end{table}

==> tex/discussion.tex <==
We modify the Decision Transformer architecture to handle environments with discrete action spaces and apply it to the
task of programmatic policy synthesis in the Karel domain. We train our model using trajectories sampled from a random
policy. Our experiments show that the model is competitive with LEAPS while requiring significantly less training data
and search over program space.

\subsection{Training Requirements}

The decision transformer model requires less training data and searches over a
smaller program space than LEAPS. LEAPS trains on 35,000 programs while the
decision transformer model requires just 500 programs to achieve the same performance.
Table~\ref{tab:dt-results} shows that LEAPS searches over a much larger number of programs for each task, compared to the 64 programs that
the decision transformer searches over.

\subsection{Sensitivity to Training Data Quality}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figs/dt_pct_traj.pdf}
    \caption{Return of the Decision Transformer model when trained on the top-$k$\% of the dataset.}
    \label{fig:dt-pct-traj}
\end{figure}

To evaluate the sensitivity of the decision transformer model to the quality of the training data, we train the model
on the top-$k$\% of trajectories by return on the \verb|topOff| task. We sample $64$ programs from the model at each time step and plot the maximum
return achieved by a program. Figure~\ref{fig:dt-pct-traj} shows that the model is highly sensitive to the quality of the
training dataset.

\subsection{Hardware Requirements}

The decision transformer model for each Karel task was trained on a compute cluster node
with an AMD Epyc Rome series CPU, 128GB RAM, and a single NVIDIA GeForce RTX
2060 Super GPU. Each model for a task took approximately 30 minutes to train.

\subsection{Reward Variance}

\com{discuss the stddev of return for programs for each model - how much reward can be expected from a program generated by each model?
Generally want to evaluate the ``brittleness'' of the model.}

\subsection{Effect of Evaluation Target}

\com{discuss how the evaluation target affects the performance of each model - ``controllability''}

\subsection{Novelty of Generated Programs}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figs/dt_similarity.pdf}
    \caption{Box plot of returns for programs sampled from the decision transformer model.}
    \label{fig:dt-similarity}
\end{figure}

To evaluate the similarity of programs generated by the decision transformer model to those in the
training dataset, we sample $998$ programs from a model trained on the \verb|topOff| task.
After de-duplication, we identify the set of novel synthesized programs ($P_\text{novel}$) that are not present in the training dataset and those that are ($P_\text{dup}$),
and plot the distribution of returns for both as a boxplot in Figure~\ref{fig:dt-similarity}.
To test the hypothesis that the mean returns of $P_\text{nov}$ is not less than that of $P_\text{dup}$, we use a one-sided Welch's t-test
due to them having unequal sample sizes ($|P_\text{nov}|=643$, $|P_\text{dup}|=115$) and variances ($\sigma^2_{nov}=8.99\times 10^{-3}$, $\sigma^2_{dup}=7.73\times 10^{-3}$).
We find that the mean return of the programs in $P_\text{dup}$ is
significantly higher ($p < 0.01$) than the mean return of the novel programs in $P_\text{nov}$. This suggests that while the decision
transformer is capable of producing novel programs, they tend to have lower return than the dataset the model was trained
on.

\subsection{Qualitative Analysis of Generated Programs}

\com{show some examples of programs generated by DT and discuss them qualitatively}

\input{figs/dt_progs.tex}

\subsection{Generalization to New Tasks}

\com{Run generalization experiments and com on results.}

==> tex/dt/preliminaries.tex <==
\subsection{Offline reinforcement learning}

We borrow the definition of a Markov decision process (MDP) from \citet{levine2020offline} as a tuple $\mathcal{M}
    \doteq (\mathcal{S}, \mathcal{A}, \mathcal{P}, d_0, r, \gamma)$, consisting of states $s_t \in
    \mathcal{S}$ that may be discrete or continuous, actions $a_t \in \mathcal{A}(s)$ which can also be discrete or
continuous, transition dynamics $\mathcal{P}(s'|s,a) \doteq \Pr\{S_t=s'|S_{t-1}=s, A_{t-1}=a\}$ that describe the
dynamics of the system, initial state distribution $d_0(s_0)$, reward function $r \in \mathcal{R}: \mathcal{S} \times
    \mathcal{A} \rightarrow \mathbb{R}$ at timestep $t$, and a scalar discount factor $\gamma \in [0, 1)$. A policy $\pi$
describes a process for selecting actions given states, thus inducing a trajectory $\tau \doteq ( s_0, a_0, \cdots,
    s_H, a_H )$, with the trajectory distribution $p_\pi (\tau) = \prod_{t=0}^{H}
    \pi(a_t|s_t)\mathcal{P}(s_{t+1}|s_t,a_t)$. The reinforcement learning objective, $J(\pi)$, can then be written as an
expectation under this trajectory distribution:

\begin{equation}
    J(\pi) \doteq \mathbb{E}_{\tau \sim p_\pi(\tau)} \left[ \sum_{t=0}^{H} \gamma^t r(s_t,a_t) \right] \label{eq:rl-objective}
\end{equation}

In offline reinforcement learning, instead of the same policy being used to explore the environment while also being
optimized, we explore the environment using a separate, fixed \textit{behavior} policy $b$, and use its experience to
optimize the target policy $\pi$~\citep{sutton2018reinforcement}.

\subsection{Transformers}

Transformers were proposed by \citet{vaswani_attention_2017} as an architecture to efficiently model sequences. They
consist of stacked self-attention layers with residual connections. Each self-attention layer receives $n$ embeddings
$\{ x_i \}_{i=1}^n$ corresponding to unique input tokens, and outputs $n$ embeddings $\{ z_i \}_{i=1}^n$, preserving the
input dimensions. The $i$-th token is mapped via linear transformations to a key $k_i$, query $q_i$, and value $v_i$.
The $i$-th output of the self-attention layer is given by weighting the values $v_j$ by the normalized dot product
between the query $q_i$ and other keys $k_j$:

\begin{equation}
    z_i = \sum_{j=1}^n \texttt{softmax} \left( \{ \left< q_i, k_{j'} \right> \}_{j'=1}^n \right)_j \cdot v_j
\end{equation}

This allows the layer to assign \enquote{credit} by implicitly forming state-return associations via similarity of the
query and key vectors (maximizing the dot product). Decision transformers use the GPT
architecture~\citep{radford2018improving}, which modifies the transformer architecture with a causal self-attention
mask to enable autoregressive generation, replacing the summation/softmax over the $n$ tokens with only the previous
tokens in the sequence $(j \in [1, i])$. We defer the other architectural details to the original papers.

\subsection{Decision Transformers}

Decision transformers were proposed by \citet{chen_decision_2021} as an architecture to apply the sequence-modeling
capabilities of transformers to sequential decision problems. Trajectories are represented as:

\begin{equation}
    \tau = \left( \widehat{R}_1, s_1, a_1, \widehat{R}_2, s_2, a_2, \cdots, \widehat{R}_T, s_T, a_T \right)
\end{equation}

where rewards are modeled as the returns-to-go $\widehat{R}_t = \sum_{t'=t}^{T} r_{t'}$. States, actions and returns are
embedded using separate, fully-connected layers. Additionally, an embedding is learned for each timestep and added to
each token. This is different from the standard positional embedding used by transformers, as one timestep corresponds
to three tokens. The tokens are then processed by a GPT~\citep{radford2018improving} model, which predicts future
actions via autoregressive modeling.

\subsection{Programmatic Policy Synthesis}

Programmatic policy synthesis is the task of learning to synthesize a program structured in a given domain-specific
language (DSL) that can be executed to solve a given task described by an MDP, purely from reward. The program $\rho$
essentially acts as a policy in the MDP. The programs, or programmatic policies, considered in this work
are defined based on a DSL shown in Figure~\ref{karel-dsl}. Formally, given a DSL $G=(V,\Sigma,R,S)$~\citep{sipser1996intro} which
defines the space of possible programmatic policies, and an MDP $\mathcal{M}_{\text{exec}}$ in which a programmatic policy $\rho$
can execute and obtain reward, we define the programmatic policy synthesis task as an MDP $\mathcal{M}_{\text{syn}}$, where:

\begin{itemize}
    \item $\mathcal{S}_{\text{syn}} \doteq \{w \in (V \cup \Sigma)^*\ |\ S \xRightarrow[]{*} w\}$ and is the current sequence
          of terminals and non-terminals in the partially expanded program $(w_0, w_1, \cdots, w_i, \cdots)$.
    \item $\mathcal{A}_{\text{syn}} \doteq R \times V \times \mathbb{N}$ and is the space of all actions consisting of applying a rule $r$ to a
          non-terminal symbol $v$ located at index $i$ in the current state. \com{Better formalization?}
    \item $\mathcal{P}_{\text{syn}}$ is the transition function which represents the deterministic transition to a state
          where the production rule has been applied to the selected non-terminal symbol if such an action was valid. If
          not, the state remains unchanged. \com{how to better formalize this?}
    \item $d_{0,\text{syn}}({S}) = 1$
    \item $r_{\text{syn}} \doteq \begin{cases} r_{\text{exec}}, & \text{if current state } s \in
              \mathcal{S}_{\text{syn}} \text{ is terminal}      \\
              0,               & \text{otherwise}\end{cases}$
    \item $\gamma_{\text{syn}} = 1$ \com{Justification?}
\end{itemize}

The goal of the programmatic policy synthesis task is to synthesize a program $\rho$ that maximizes the objective function $J(\rho)$ which is defined similarly as in Equation~\ref{eq:rl-objective}.

\input{figs/karel-dsl.tex}
